Serendipitous Nebular-phase JWST Imaging of SN Ia 2021aefx: Testing the Confinement of 56-Co Decay Energy

We present new 0.3-21 micron photometry of SN 2021aefx in the spiral galaxy NGC 1566 at +357 days after B-band maximum, including the first detection of any SN Ia at >15 micron. These observations follow earlier JWST observations of SN 2021aefx at +255 days after the time of maximum brightness, allowing us to probe the temporal evolution of the emission properties. We measure the fraction of flux emerging at different wavelengths and its temporal evolution. Additionally, the integrated 0.3-14 micron decay rate of $\Delta m_{0.3-14} = 1.35 \pm 0.05$ mag/100 days is higher than the decline rate from the radioactive decay of $^{56}$Co of $\sim 1.2$mag/100 days. The most plausible explanation for this discrepancy is that flux is shifting to >14 micron, and future JWST observations of SNe Ia will be able to directly test this hypothesis. However, models predicting non-radiative energy loss cannot be excluded with the present data.

==> fn1.tex <==
%footnote
This does not account for flux emerging at $>14~\um$.
